Fin-RSI: A Unified Library of Financial Skills, Checks, and Self-Improvement for LLM Agents

As large language models (LLMs) become more capable, financial agents need tools they can readily discover and use. Yet financial software is fragmented across libraries with different interfaces and conventions, making it difficult to build reliable agent workflows. We present Fin-RSI, a unified Python library of financial skills, checks, and self-improvement designed for LLM agents. It brings together tools for market analysis, forecasting, portfolio construction, and trading research through shared interfaces across models and agent frameworks. Agents can find suitable tools from natural-language requests, reuse tested implementations, and improve generated programs through checking and feedback. Developers can extend the library with new tools without rebuilding integrations for each model. Across 20 open-weight models on six trading-position tasks, tool discovery increased the proportion of episodes producing valid programs from 9.7% to 29.2%; for models with at least 14 billion parameters, it rose from 23.6% to 64.6%. We release the library and benchmark as a shared resource for the community and plan to expand its tools and task coverage as financial agents evolve.

==> shared/figures/episode_lag.tex <==
\def\LagK{8}%
\def\LagRows{17}%
\def\LagCellsA{0,0,0,0,0,0,0,0,0,1,1,1,1,1,1,1,1}%
\def\LagCellsB{0,0,0,0,0,0,0,0,2,1,1,1,1,1,1,1,1}%


==> shared/figures/glyphs.tex <==
\ifcsname figTitleFont\endcsname\else\InputIfFileExists{figures/figstyle}{}{\input{shared/figures/figstyle}}\fi%
\providecommand{\gpage}[4]{%
  \begin{scope}[shift={#1}]%
    \path[fill=#4, draw=gline, line width=0.5pt, line join=round, gshade]%
      ({-#2/2},{-#3/2}) -- ({#2/2},{-#3/2}) -- ({#2/2},{#3/2-0.2}) -- ({#2/2-0.2},{#3/2}) -- ({-#2/2},{#3/2}) -- cycle;%
    \draw[gline, line width=0.5pt, line join=round, fill=gline!40] ({#2/2-0.2},{#3/2}) -- ({#2/2-0.2},{#3/2-0.2}) -- ({#2/2},{#3/2-0.2});%
  \end{scope}}%
\providecommand{\gbar}[4]{\draw[#4, line width=2.4pt, line cap=round] (#1,#2) -- ({#1+#3},#2);}%
\providecommand{\gcheck}[2]{%
  \ifnum#2=1 \fill[figok] #1 circle (0.13);%
    \pic[draw=white, line width=0.85pt, scale=0.62] at #1 {lu check};%
  \else \fill[figbad] #1 circle (0.13);%
    \pic[draw=white, line width=0.85pt, scale=0.62] at #1 {lu x};\fi}%
\providecommand{\gcard}[1]{%
  \begin{scope}[shift={#1}]%
    \path[fill=finblue!12, draw=finblue!70, line width=0.55pt, fig item, gshade] (-0.22,-0.16) rectangle (0.22,0.16);%
    \draw[finblue!70, line width=0.9pt, line cap=round] (-0.13,0.05) -- (0.13,0.05) (-0.13,-0.05) -- (0.06,-0.05);%
  \end{scope}}%
\providecommand{\glock}[1]{%
  \fill[white] #1 circle (0.19);%
  \pic[draw=figink!80, line width=0.95pt, scale=1.05] at #1 {lu lock};}%
\providecommand{\gbot}[2]{%
  \path[fill=figink, fig shadow] #1 circle (#2);%
  \pic[draw=white, line width=0.75pt, scale={4.2*#2}] at #1 {lu bot};}%

